FAHT: An Adaptive Fairness-aware Decision Tree Classifier

Automated data-driven decision-making systems are ubiquitous across a wide spread of online as well as offline services. These systems, depend on sophisticated learning algorithms and available data, to optimize the service function for decision support assistance. However, there is a growing concern about the accountability and fairness of the employed models by the fact that often the available historic data is intrinsically discriminatory, i.e., the proportion of members sharing one or more sensitive attributes is higher than the proportion in the population as a whole when receiving positive classification, which leads to a lack of fairness in decision support system. A number of fairness-aware learning methods have been proposed to handle this concern. However, these methods tackle fairness as a static problem and do not take the evolution of the underlying stream population into consideration. In this paper, we introduce a learning mechanism to design a fair classifier for online stream based decision-making. Our learning model, FAHT (Fairness-Aware Hoeffding Tree), is an extension of the well-known Hoeffding Tree algorithm for decision tree induction over streams, that also accounts for fairness. Our experiments show that our algorithm is able to deal with discrimination in streaming environments, while maintaining a moderate predictive performance over the stream.

==> FAHT_An Adaptive Fairness_aware Decision Tree Classifier/related.tex <==
Relevant to our work is work on fairness-aware learning as well as works on stream learning, in particular stream classification with decision tree models.

\subsection{Fairness-aware Learning}
A number of research approaches have been proposed to address the problem of bias and discrimination in machine learning systems due to the inherent bias in data and the complex interaction between data and learning algorithms~\cite{pedreshi2008discrimination,zliobaite2015survey,hajian2016algorithmic}. 
These approaches generally fall into one of the following categories: i) pre-processing approaches, ii) in-processing approaches and iii) post-processing approaches.


\emph{Pre-processing approaches} modify the data distribution to ensure a fair representation of the different communities (i.e., DR, DG, FR, FG) in the training set. The rationale for these approaches is that if a classifier is trained on discrimination-free data, its predictions will not be discriminatory (such a property however, cannot be guaranteed). 
A popular method in this category is massaging~\cite{kamiran2009classifying} that swaps the class labels of selected instances to restore balance. A ranker is used to carefully select the instances to be swapped in order to minimize the effect of label swapping on predictive accuracy; these are the instances closest to the decision boundary. 
Instead of intrusively relabeling the instances, reweighting~\cite{calders2009building} assigns different weights to different communities to alleviate the bias towards favored communities for the sake of benefiting the classification of deprived communities. The weights are assigned based on the expected and observed probability of an instance according to its sensitive attribute value and class. A higher weight will be assigned if the observed probability is lower than the expected probability to neutralize the discrimination. 
We emphasize that pre-processing approaches are not effective in eliminating discrimination arising from the learning algorithm itself. 

\emph{In-processing approaches} modify existing learning algorithms to also account for fairness instead of only predictive performance. Therefore, distinct from the first strategy which is classifier-agnostic, these approaches are algorithm-specific. 
For example, \cite{aghaei2019learning} added regularization terms to the Mixed-Integer Programming model to penalize discrimination. \cite{calders2010three} proposes three approaches for fairness-aware Naïve Bayes classifiers: the first one alters the decision distribution until there is no more discrimination, the second one attempts to remove the correlation between sensitive attribute and class label by building a separate model for each sensitive group, and the third one models a latent variable to discover the actual class labels of a discrimination-free dataset. 
Closer to our work is the work  by~\cite{kamiran2010discrimination} that incorporates discrimination into the splitting criterion of a decision tree classifier. Two key distinctions are: i) fairness in our work is directly defined in terms of the discrimination difference of the induction of a split, i.e., the fairness gain due to the split rather than the entropy w.r.t. sensitive attribute and ii) our model operates in an online setting rather than upon a static/batch dataset. The online learning scenario is much more challenging as decisions have to be made without access to the complete dataset and moreover, such decisions have an impact on following decisions in terms of both accuracy and fairness (feedback loops). 


Finally, \emph{post-processing approaches} modify the resulting models by ``correcting'' the decision regions that lead to redlining for a fair representation of different subgroups in the final decision process. In~\cite{hajian2015discrimination}, the fair patterns are processed with $k$-anonymity to work against discrimination.  \cite{kamiran2010discrimination} carefully relabels selected leaves of a decision tree model to reduce  discrimination with the least possible impact on accuracy.
Transferring such approaches to a stream setting is not straightforward as the decision regions/leaves might change over the course of the stream due to concept drifts.
%As the decision regions in a data stream environment are not stable but rather might change with time, this method is not applicable to our learning settings.


\subsection{Stream Classification}
The main challenge for learning in a stream environment is the so called, concept-drifts, i.e., changes in the joint data distribution over time~\cite{krawczyk2017ensemble,aggarwal2007data,gama2014survey}. The learning methods therefore should be able to adapt to changes by learning incrementally from new instances, e.g.,~\cite{oza2005online,zhang2017hybrid} and by carefully considering historical information into the model by e.g., forgetting outdated information, e.g.,~\cite{melidis2018learning,wagner2015ageing} and/or focusing on most recent data, e.g.,~\cite{bifet2007learning}
%The adaption strategy in literature falls broadly in three categories: i) sliding window techniques use the most recent examples to build a model in order to update the knowledge from new data~\cite{bifet2007learning}; ii) online methods learn incrementally based on new instances from the stream~\cite{oza2005online}; iii) an ensemble of classifiers produce outputs of several classifiers and modify ensemble components or their aggregation to adapt to changes~\cite{kuncheva2004classifier}. 

%The adaption strategy in literature falls broadly in three categories: 1) sliding window techniques use the most recent examples to build a model in order to update the knowledge from new data~\cite{bifet2007learning}; 2) online methods learn incrementally based on new instances from the stream~\cite{oza2005online}; 3) an ensemble of classifiers produce outputs of several classifiers and modify ensemble components or their aggregation to adapt to changes~\cite{kuncheva2004classifier}. 


Our approach integrates the algorithm-level solution for fairness-aware classification and the online approach to maintain an accurate and up-to-date classifier for infinite data streams with non-stationary distribution and discrimination bias. We build our model on top of the Hoeffding tree~\cite{domingos2000mining}, one of the most popular decision tree classifiers for data streams. Hoeffding tree relies on the Hoeffding bound to make confident decisions about the selection of splitting attributes over infinitive streams and accommodates new instances from the stream incrementally. 
To enable fairness-aware learning, we revise the learning model by not only incorporating new examples from the stream but also by alleviating their bias towards the favoured group through a new splitting criterion, the \emph{fair information gain}, that jointly considers the information and the fairness gain of a split.

